Opaque Response Generation Enabling Automatic Creation of Virtual Services for Service Virtualisation

Service virtualisation is a method to create virtual service models that can mimic interaction behaviors between a system under test and the target system. With service virtualisation, the development team can get access to the production-like conditions whenever and however many times they need, enabling frequent and comprehensive testing. Previous techniques for service virtualisation have relied on explicitly modelling the target services by a service expert and require detailed knowledge of message protocol and structure. However, neither of these are necessarily available. In this thesis, we introduce our novel opaque response generation approach. This approach enables services to be virtualised automatically without any expert knowledge or documentation of system protocol and interaction behaviours. Given a collection of interactions exchanged between a system under test and a target real service, our approach can 1) organise the same type of interactions into the same cluster and derive a cluster prototype for each cluster; 2) search a given incoming request for its the most similar request in the interaction library; 3) learn knowledge from the incoming request and the recorded interaction; and 4) generate a response. A framework and proof-of-concept implementation of our opaque response generation approach is described. Experimental results show our opaque response generation approach is able to automatically generate accurate responses in real time with an accuracy rate over 99% on average.

==> abstract.tex <==
\cleardoublepage

\Large \textbf{Abstract}
\normalsize
%highly interconnected software environment, developmenDataMiningt constrains in software development circle
% quality software deliver on time , modern software relies on other systems

Nowadays, an enterprise system interacts with many other systems to perform functionalities. With the trend of ever increasing inter-connectedness between software systems, one of the primary obstacles facing today's software development teams is the ability to develop and test a software system independent of the other systems on which it depends. Replicating a production environment for testing is expensive, time-consuming and error-prone. Moreover, software developers will usually have only limited access to it. However, continuous access to production-like conditions to test their application is an important part of the modern development method {\em Development-Operations (known as `DevOps')}. Service virtualisation technique can make continuous access into a reality.
%Getting access to the actual production environment for testing is not possible due to the risk of disruption. Large organisations often have a test environment, which is a close replication of their production environment, but this is very expensive. Furthermore the test environment is in high demand, so software developers will have only limited access to it.

Service virtualisation is a method to create virtual service models that can mimic interaction behaviors between a system under test and the target system. With service virtualisation, the development team can get access to the production-like conditions whenever and however many times they need, enabling frequent and comprehensive testing. Previous techniques for service virtualisation have relied on explicitly modelling the target services by a service expert and require detailed knowledge of message protocol and structure. However, neither of these are necessarily available.

In this thesis, we introduce our novel opaque response generation approach. This approach enables services to be virtualised automatically without any expert knowledge or documentation of system protocol and interaction behaviours. Given a collection of interactions exchanged between a system under test and a target real service, our approach can 1) organise the same type of interactions into the same cluster and derive a cluster prototype for each cluster; 2) search a given incoming request for its the most similar request in the interaction library; 3) learn knowledge from the incoming request and the recorded interaction; and 4) generate a response. A framework and proof-of-concept implementation of our opaque response generation approach is described. Experimental results show our opaque response generation approach is able to automatically generate accurate responses in real time with an accuracy rate over 99\% on average.

\clearpage 

==> experiment.tex <==
\chapter{Experiment}
